360+x: A Panoptic Multi-modal Scene Understanding Dataset

Human perception of the world is shaped by a multitude of viewpoints and modalities. While many existing datasets focus on scene understanding from a certain perspective (e.g. egocentric or third-person views), our dataset offers a panoptic perspective (i.e. multiple viewpoints with multiple data modalities). Specifically, we encapsulate third-person panoramic and front views, as well as egocentric monocular/binocular views with rich modalities including video, multi-channel audio, directional binaural delay, location data and textual scene descriptions within each scene captured, presenting comprehensive observation of the world. Figure 1 offers a glimpse of all 28 scene categories of our 360+x dataset. To the best of our knowledge, this is the first database that covers multiple viewpoints with multiple data modalities to mimic how daily information is accessed in the real world. Through our benchmark analysis, we presented 5 different scene understanding tasks on the proposed 360+x dataset to evaluate the impact and benefit of each data modality and perspective in panoptic scene understanding. We hope this unique dataset could broaden the scope of comprehensive scene understanding and encourage the community to approach these problems from more diverse perspectives.

==> asset/table/ssl+cls.tex <==



\begin{table}[!t]
% \begin{minipage}{.39\textwidth}
% \begin{table*}
	\centering
	\caption{Models with different pre-train methods were fine-tuned and tested on video classification. The experiments use all three video views. Reported in Avg. Prec. (\%). }
\label{tab:ssl+cls}
%     % \hspace{0.2pt}
% 	\small
% 	% \setlength{\tabcolsep}{4pt}
\resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}l|ccc@{}}
     \toprule
   \multirow{2}{*}{ Pre-train Method } &   \multicolumn{3}{c}{Modalities}  \\
     & V & V + A & V + A + D  \\
      \midrule
      % \pm
      From Scratch &
     63.73 \e{0.0} & 77.32 \e{0.0} & 80.62 \e{0.0} 
      %& \multirow{3}{*}{360$^{\circ}$  + Front +  Binocular}
     \\  
        
      % \midrule
      Video Pace~\cite{Wang20} & 69.27 \p{5.5} & 79.56 \p{2.2} & 81.97 \p{1.3} \\  
 
      % \midrule
    Clip Order~\cite{xu2019self} & 69.91 \p{6.2} & 80.14 \p{2.8} & 82.18 \p{1.6} \\  

      % \midrule
       % Video Pace + Clip Order 
       VP~\cite{Wang20} + CO~\cite{xu2019self}
     & \boldsymbol{$76.84$~\p{13.1}} & \boldsymbol{$82.66$~\p{5.3}} & 
     \boldsymbol{$83.32$~\p{2.7}}\\
      % \midrule
     \bottomrule
    \end{tabular}
    }

% \vspace{-2mm}
\end{table}
% \hfill


==> asset/table/ssl+tal.tex <==

\begin{table}[!t]
% \begin{minipage}{.5\textwidth}
% \begin{table*}
	\centering
	 \caption{Comparison between supervised pre-trained extractors with SSL pre-trained counterparts on TAL task. The experiments use all three video views with modalities (V+A+D). }
\label{tab:ssl+tal}
%     % \hspace{0.2pt}
% 	\small
% 	% \setlength{\tabcolsep}{4pt}
% % \hspace*{-1.0cm}
\resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}l|ccc|c@{}}
     \toprule
      \makecell[l]{Pre-train Method}
      & \makecell[c]{mAP\\$@$0.5} & \makecell[c]{mAP\\$@$0.75} & \makecell[c]{mAP\\$@$0.95} & Avg.  \\
      \midrule
       Supervised
       & $27.1$ \e{0.0} & $18.7$ \e{0.0} & $7.0$ \e{0.0} & $17.6$ \e{0.0}   \\
       % \midrule
       Video Pace~\cite{Wang20}
       & $29.4$ \p{2.3} & $19.6$\p{0.9} & $7.4$\p{0.4} & $18.8$ \p{1.2}  \\
        % \midrule
   Clip Order~\cite{xu2019self}
       &$28.9$ \p{1.8}& $19.3$ \p{0.6}& $7.3$ \p{0.3}& $18.5$ \p{0.9} \\
        % \midrule 
     % Video Pace + Clip Order 
    VP~\cite{Wang20} + CO~\cite{xu2019self}
       &\boldsymbol{ $30.3$ }\p{3.2}& \boldsymbol{$20.2$}\p{1.5} & \boldsymbol{$7.9$}\p{0.9} & \boldsymbol{$19.5$~\p{1.9}}  \\
     \bottomrule
    \end{tabular}
    }
% \vspace{-1mm}
\end{table}



==> asset/table/ssl.tex <==

\begin{table*}[!h]
	\caption{Models pre-trained with different self-supervise methods were tested on video classification. The methods use all three video types together.}
    % \hspace{0.2pt}
	\small
	\centering
	\setlength{\tabcolsep}{4pt}

    \begin{tabular}{c|c|c}
     \toprule
 
    Pre-trained Method &  Modalities  &  Avg. Precision (\%) $ \ \pm\  $ STD \\
      \midrule

      
      \multirow{3}{*}{From Scratch} %& \multirow{3}{*}{360$^{\circ}$  + Front +  Binocular}
      &   V   &          $ 0.72 \ \pm \ 0.027  $  \e{0.00} \\  
      & V + A &        $ 0.83\  \pm\  0.027  $   \e{0.00}   \\
      & V + A + D  &   $ 0.89 \ \pm \ 0.022  $  \e{0.00}    \\
      \midrule
      
      \multirow{3}{*}{Video Pace} %&& \multirow{3}{*}{360$^{\circ}$  + Front +  Binocular}
      &   V   &          $ 0.80 \ \pm \ 0.025  $   \p{0.08} \\  
      & V + A &        $ 0.86\  \pm\  0.023  $    \p{0.03}  \\
      & V + A + D  &   $ 0.93 \ \pm \ 0.020  $     \p{0.04} \\
      \midrule

    \multirow{3}{*}{Video Clip Order} %&& 
    % \multirow{3}{*}{360$^{\circ}$  + Front +  Binocular}
      &   V   &          $ 0.82 \ \pm \ 0.024  $   \p{0.10}\\  
      & V + A &        $ 0.87\  \pm\  0.023  $    \p{0.04}  \\
      & V + A + D  &   $ 0.93 \ \pm \ 0.019  $     \p{0.04} \\
      \midrule

     \multirow{3}{*}{\makecell[c]{   Video Pace\\+\\Video Clip Order    }}  
    % \multirow{3}{*}{360$^{\circ}$  + Front +  Binocular} 
      &   V   &          $ 0.88 \ \pm \ 0.022  $   \p{0.16} \\  
      &  V + A &        $ 0.91\  \pm\  0.021  $   \p{0.08}   \\
      &  V + A + D  &   $ 0.96 \ \pm \ 0.015  $     \p{0.07} \\
      % \midrule
      
      
   
     \bottomrule
    \end{tabular}
% \vspace{-0.1cm}
\label{tab:ssl}
\end{table*}







==> asset/table/tal2.tex <==

% \hspace{-2cm}

\begin{table*}[!t]
	 \caption{Comparison between supervised pre-trained extractors with SSL pre-trained counterparts for temporal action localization.}
    % \hspace{0.2pt}
	\small
	\centering
	\setlength{\tabcolsep}{4pt}

% \hspace*{-1.0cm}
    \begin{tabular}{c|c|c|c|c|c}
     \toprule
 
      Pre-training Method &   Modalities  & mAP$@$0.5 & mAP$@$0.75 & mAP$@$0.95& Avg.  \\
      \midrule
              
    \multirow{3}{*}{\makecell[c]{Supervised
    Baseline\\Extractors }} 
       & V   &           $18.4 $    & $ 10.8$    &  $3.3$   &  $10.8$\e{0.00}    \\  
       & V + A&     $23.6$      &  $16.2$    & $5.2$   &  $15.0$\e{0.00}  \\         
       & V + A + D  & $25.9$     &   $17.8$                   &   $5.3$      &   $16.3$\e{0.0}  \\

       \midrule
      
      \multirow{3}{*}{\makecell[c]{  Video Pace     }} 
       & V   &     $ 24.4   $            &   $14.9$                 &    $6.6$  & $15.3$\p{4.5} \\  
       & V + A&     $28.7  $        &   $18.2$                  &    $7.1$   &  $18.0$\p{3.0} \\  
       & V + A + D  & $30.9$     &   $20.8$                   &     $7.5$  & $19.7$\p{3.4}  \\
        \midrule

    \multirow{3}{*}{\makecell[c]{  Video Clip Order     }} 
       & V   &        $ 24.6   $            &   $15.2$         &    $6.7$  & $15.5$\p{4.7} \\  
       & V + A&     $ 28.5  $        &   $18.0$              &    $7.0$   &  $17.8$\p{2.8} \\  
       &  V + A + D  & $30.2$     &   $19.9$                  &   $7.3$  & $19.1$\p{2.8}  \\
        \midrule 

        
    \multirow{3}{*}{\makecell[c]{  Video Pace\\+\\Video Clip Order       }} 
       & V   &     $ 25.5   $            &   $18.0$               &    $7.4$  & $17.0$\p{6.2} \\  
       &  V + A&     $29.4  $        &   $20.2$                  &    $8.0$   &  $19.2$\p{4.2} \\  
       &  V + A + D  & $31.1$     &   $20.5$                     &    $8.4$  & $20.0$\p{4.7}  \\
        % \midrule 

        
    % \multirow{3}{*}{\makecell[c]{  Video Pace\\+\\Video Clip Order       }} 
    % % & \multirow{3}{*}{ \makecell[c]{  Video Classification       } } 
    %    & V   &     $ 28.2   $            &   $19.7$                          &    $7.9$         & $18.6$\p{7.8} \\  
    %    &  V + A&     $33.8  $        &   $22.3$                             &    $8.7$           &  $21.6$\p{6.6}  \\  
    %    &  V + A + D  & $\boldsymbol{34.6}$     &   $\boldsymbol{22.8}$      &   $\boldsymbol{9.2}$  & $\boldsymbol{22.2}$\p{5.9}  \\
       
     \bottomrule
    \end{tabular}
\vspace{-0.1cm}
\label{tab:tal2}
\end{table*}




% % \hspace{-2cm}

% \begin{table*}[!t]
% 	 \caption{\textbf{Temporal action localization result.} The first-stage feature extractors were pre-trained and subsequently fine-tuned using designated methods.}
%     \hspace{0.2pt}
% 	\small
% 	\centering
% 	\setlength{\tabcolsep}{4pt}

% \hspace*{-1.0cm}
%     \begin{tabular}{c|c|c|c|c|c|c}
%      \toprule
 
%       Pre-training Method &  Fine-tuning Method  & Modalities  & mAP$@$0.5 & mAP$@$0.75 & mAP$@$0.95& Avg.  \\
%       \midrule
              
%     \multirow{3}{*}{\makecell[c]{ From Scratch       }} & \multirow{3}{*}{ \makecell[c]{  Video Classification       } } 
%        & V   &     $ 25.8   $            &   $17.7$               &    $6.8$   & $16.8$\e{0.0} \\  
%        & & V + A&     $30.1  $        &   $20.4$                  &    $7.5$   &  $19.3$\e{0.0} \\  
%        & & V + A + D  & $32.4$     &   $21.1$                   &   $7.8$      &   $20.4$\e{0.0}  \\

%        \midrule
      
%       \multirow{3}{*}{\makecell[c]{  Video Pace     }} & \multirow{3}{*}{ ---   } 
%        & V   &     $ 24.4   $            &   $14.9$                 &    $6.6$  & $15.3$\m{1.5} \\  
%        & & V + A&     $28.7  $        &   $18.2$                  &    $7.1$   &  $18.0$\m{1.3} \\  
%        & & V + A + D  & $30.9$     &   $20.8$                   &     $7.5$  & $19.7$\m{0.7}  \\
%         \midrule

%     \multirow{3}{*}{\makecell[c]{  Video Clip Order     }} & \multirow{3}{*}{  ---   } 
%        & V   &        $ 24.6   $            &   $15.2$         &    $6.7$  & $15.5$\m{1.3} \\  
%        & & V + A&     $ 28.5  $        &   $18.0$              &    $7.0$   &  $17.8$\m{1.5} \\  
%        & & V + A + D  & $30.2$     &   $19.9$                  &   $7.3$  & $19.1$\m{1.3}  \\
%         \midrule 

        
%     \multirow{3}{*}{\makecell[c]{  Video Pace\\+\\Video Clip Order       }} & \multirow{3}{*}{  ---   } 
%        & V   &     $ 25.5   $            &   $18.0$               &    $7.4$  & $17.0$\p{0.2} \\  
%        & & V + A&     $29.4  $        &   $20.2$                  &    $8.0$   &  $19.2$\m{0.1} \\  
%        & & V + A + D  & $31.1$     &   $20.5$                     &    $8.4$  & $20.0$\m{0.4}  \\
%         \midrule 

        
%     \multirow{3}{*}{\makecell[c]{  Video Pace\\+\\Video Clip Order       }} & \multirow{3}{*}{ \makecell[c]{  Video Classification       } } 
%        & V   &     $ 28.2   $            &   $19.7$                          &    $7.9$         & $18.6$\p{1.8} \\  
%        & & V + A&     $33.8  $        &   $22.3$                             &    $8.7$           &  $21.6$\p{2.3}  \\  
%        & & V + A + D  & $\boldsymbol{34.6}$     &   $\boldsymbol{22.8}$      &   $\boldsymbol{9.2}$  & $\boldsymbol{22.2}$\p{1.8}  \\
       
%      \bottomrule
%     \end{tabular}
% \vspace{-0.1cm}
% \label{tab:tal2}
% \end{table*}






% \hspace{-2cm}

% \begin{table*}[!ht]
% 	 \caption{\textbf{Temporal action localization result.} The feature extractors are pretrained using \textit{video pace + clip order} method on video classification task.}
%  % \multirow{3}{*}{360$^{\circ}$  + Front +  Binocular}
%     \hspace{0.2pt}
% 	\small
% 	\centering
% 	\setlength{\tabcolsep}{4pt}

% \hspace*{-1.2cm}
%     \begin{tabular}{c|cc|c|c|c}
%      \toprule
 
%     Pre-trained Method & \multicolumn{2}{c}{Pre-trained Datasets}   & Modalities  & Top-1 Accuracy (\%) & Top-5 Accuracy (\%) \\
%       \midrule
      
%        \multirow{3}{*}{\makecell[c]{  Supervised with \\ Video Classification    }}  &  \multirow{3}{*}{\makecell[c]{ Video: \\Audio: \\Directional: }}  &  \multirow{3}{*}{\makecell[c]{  Kinetics 400 \cite{carreira2018quo}\\AudioSet \cite{audioset}\\360+X}}  
%       & V   &                        \\  
%        & & & V + A&                        \\  
%        & & & V + A + D  & -  & -\\
%       \midrule
      
%      \multirow{3}{*}{\makecell[c]{  Supervised with \\ Video Classification    }} & \multirow{3}{*}{\makecell[c]{ Video: \\Audio: \\Directional: }}  &  \multirow{3}{*}{\makecell[c]{  360+X\\360+X\\360+X}}
%        & V   &                        \\  
%        & & & V + A&                        \\  
%        & & & V + A + D  & -  & -\\

   
%      \bottomrule
%     \end{tabular}
% \vspace{-0.1cm}
% \label{tab:tal}
% \end{table*}












% % \hspace{-2cm}

% \begin{table*}[!h]
% 	 \caption{\textbf{Temporal action localization result.} The feature extractors are pretrained using \textit{video pace + clip order} method on video classification task.}
%  % \multirow{3}{*}{360$^{\circ}$  + Front +  Binocular}
%     \hspace{0.2pt}
% 	\small
% 	\centering
% 	\setlength{\tabcolsep}{4pt}

% \hspace*{-1.2cm}
%     \begin{tabular}{c|c|c|c|c}
%      \toprule
 
%     Pre-trained Method & Pre-trained Datasets   & Modalities  & Top-1 Accuracy (\%) & Top-5 Accuracy (\%) \\
%       \midrule
      
%        \multirow{3}{*}{\makecell[c]{  Supervised with \\ Video Classification    }}  &  \multirow{3}{*}{\makecell[c]{ Video: Kinetics 400 \cite{carreira2018quo}\\Audio: AudioSet \cite{audioset}\\Directional: 360+X}}  
%       & V   &                        \\  
%       & & V + A&                        \\  
%       & & V + A + D  & -  & -\\
%       \midrule
      
%       \multirow{3}{*}{Video Pace} & \multirow{3}{*}{All: 360+X} 
%       & V&                        \\  
%       & & V + A&                        \\  
%       & & V + A + D&                        \\  
%       \midrule

%     \multirow{3}{*}{Video Clip Order} & \multirow{3}{*}{All:360+X}  
%       & V&                        \\  
%       & & V + A&                        \\  
%       & & V + A + D&                        \\  
%       \midrule
      
%     \multirow{3}{*}{\makecell[c]{   Video Pace\\+\\Video Clip Order    }} &  
%     \multirow{3}{*}{\makecell[c]{  Video: Kinetics 400 \cite{carreira2018quo}\\Audio: AudioSet \cite{audioset}\\Directional: 360+X }}  
%       & V&                        \\  
%       & & V + A&                        \\  
%       & & V + A + D&                        \\  
    
%     \midrule
    
%     \multirow{3}{*}{\makecell[c]{   Video Pace\\+\\Video Clip Order    }} & \multirow{3}{*}{All: 360+X} 
%       & V&                        \\  
%       & & V + A&                        \\  
%       & & V + A + D&                        \\  
 


% % ---------------------- Color ------------------------------
%    % \midrule



   
%      \bottomrule
%     \end{tabular}
% \vspace{-0.1cm}
% \label{tab:tal}
% \end{table*}







==> asset/vis/on_boxes.tex <==

\begin{figure*}
    \centering 
   % L D R U
  \begin{subfigure}[b]{0.33\textwidth}   % 0.385
     \hspace{-0.9cm}
     \includegraphics[width=1.25\textwidth]{asset/img/analysis/Categories.pdf}
    % \hspace{-0.3cm}
    \caption{Distribution of the scene categories (number)}
    \label{fig:categories}
  \end{subfigure}
% --------------------------
 \hfill
    \begin{subfigure}[b]{0.33\textwidth}  % 25   0.27
    \vspace*{-20cm}
    % \vspace*{-2cm}
      % \begin{minipage}{\textwidth}
        \includegraphics[width=1.1\textwidth, clip]{rebuttal/city-action-distribution.pdf}
            \centering 
\caption{Geographical distribution of actions.}
    \label{fig:geometry}
  \end{subfigure}
% ----------------------------------------
  \hfill
  \begin{subfigure}[b]{0.33\textwidth}   % 34
   % \vspace{-5cm}
   \hspace{0.5cm}
   % L D R U
    \includegraphics[width=0.97\textwidth, trim=10 25 88 27, clip]{asset/img/analysis/labels.pdf}
     % \centering 
     { \flushright
    \caption{Overall distribution of action durations.}
        \label{fig:labels}
    }
  \end{subfigure}
 % ---------------------------------------- 
    \centering
    \hfill
  \begin{subfigure}[b]{0.33\textwidth}
    \includegraphics[width=\textwidth]{asset/img/analysis/num_of_action.pdf}
    \caption{Distribution comparison of the number of action instances per video.}
    % between existing datasets (e.g. UCF101 \cite{soomro2012ucf101}, Kinetics \cite{kay2017kinetics}, HMDB51 \cite{Kuehne11}, Ego4D \cite{grauman2022ego4d}, ActivityNet \cite{caba2015activitynet}, HACS \cite{zhao2019hacs}) and Ours.}
    \label{fig:comparison_dataset}
  \end{subfigure}
      \hfill
 \begin{subfigure}[b]{0.39\textwidth}
   \vspace*{-2mm}
    \includegraphics[width=\textwidth]{asset/img/analysis/at_statistics.pdf}
    \vspace{0.5mm}
    \caption{Binaural delay per clip}
    \label{fig:at_statistic}
  \end{subfigure}
  \hfill
         % \includegraphics[width=\textwidth, trim=0 20 0 0, clip]{asset/img/analysis/timeofday.pdf}
         % \includegraphics[width=\textwidth, trim=0 20 0 0, clip]{asset/img/analysis/timeofday.pdf}
    % \includegraphics[width=\textwidth]{asset/img/analysis/at_statistics.pdf}
    % \caption{Binaural delay per clip}
    % \label{fig:at_statistic}
        % \vspace{0.5mm}
        % \caption{Capture time of the day}
        % \label{fig:timeofday}
  % \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.27\textwidth} 
     \vspace*{-2mm}
    % \end{minipage}
     \includegraphics[width=\textwidth]{asset/img/analysis/at_statistics_distribution.pdf}
     \vspace{0.5mm}
    \caption{Overall binaural delay histogram}
    \label{fig:at_statistic_distribution}
  \end{subfigure}
  \caption{\textbf{Dataset statistics analysis}, on the distributions of (a) the scene category, (b) temporal action instance duration, (c) capturing time, and (d) number of actions per video, (e) binaural delay per clip, (f) the overall clips binaural delay.}
  \label{fig:TSL and complexity}
  \vspace{-3mm}
\end{figure*}



% \begin{figure*}
%     \centering 

%   \begin{subfigure}[b]{0.58\textwidth}
%      % \hspace{-0.9cm}
%      \includegraphics[width=\textwidth]{asset/img/analysis/Categories.pdf}
%     % \hspace{-0.3cm}
%     \caption{Video counts of scene categories }
%     \label{fig:tsl}
%   \end{subfigure}
%     \begin{subfigure}[b]{0.3\textwidth}
%     \hspace*{0.5cm}
%     \includegraphics[width=\textwidth]{asset/img/analysis/new_num_of_action.png}
%     \caption{Distribution comparison of the number of action instances per video between existing datasets (e.g. UCF101 \cite{soomro2012ucf101}, Kinetics \cite{kay2017kinetics}, HMDB51 \cite{Kuehne11}, Ego4D \cite{grauman2022ego4d}, ActivityNet \cite{caba2015activitynet}, HACS \cite{zhao2019hacs}) and Ours.}
%     \label{fig:complexity}
%   \end{subfigure}
%   \hfill
%     \begin{subfigure}[b]{0.5\textwidth}
%     \includegraphics[width=\textwidth]{asset/img/analysis/labels.pdf}
%     \caption{Duration of Action Instances}
%     \label{fig:complexity}
%   \end{subfigure}
% \begin{subfigure}[b]{0.38\textwidth}
%     \hspace*{0.5cm}
%     \includegraphics[width=\textwidth]{asset/img/analysis/timeofday.pdf}
%     \caption{Capture time of the day}
%     \label{fig:complexity}
%   \end{subfigure}

%   \centering


%   \caption{Visialisation of Dataset Analysis}
%   \label{fig:TSL and complexity}
% \end{figure*}

==> rebuttal/Answer.tex <==
\newcounter{num}
\setcounter{num}{1}

% \noindent{\bf \Rone Q\thenum: Lack of Motivation for Setup Choices: The paper could benefit from a clearer explanation of the practical scenarios where the combination of the different views.}

% Lack of Motivation for Setup Choices: 
\noindent{\bf \Rone Q\thenum: The paper could benefit from a clearer explanation of the practical scenarios where the combination of the different views would be realistically utilized.}
\vspace{0.1cm}
 % 

\noindent{\bf A:}
\stepcounter{num}
Cross-view (360°, egocentric, third-person)  understanding is essential for building interactive systems such as virtual reality (VR) and autonomous systems like agent navigation. For example, the \du~view is widely used in the construction of VR environments [Wu et al. 2020, Xiao et al. 2017, Hou et al. 2018], and the egocentric view is essential for human-centred interaction within VR. Agent navigation systems also greatly benefit from the integration of both egocentric and infrastructure-side (third-person) views to avoid occlusion [Jangir et al. 2021, Bajcsy et al. 1988, Wilkes and Tsotsos 1994]. 


% For example, current 


% While  the existing research on human interaction within VR environment, particularly in-the-wild, is limited due to the lack of available datasets. To bridge this research gap, we present a dataset that includes a human-centered perspective alongside the \du view toenables further  and other human-centered scene understanding tasks.


% While our dataset can potentially enhance research progress in the field of human-centered tasks, VR. 


 
\vspace{0.1cm}






% Our dataset is also applicable for enhancing virtual reality (VR) environments where 360° panoramic data is widely used to construct VR settings. In the creation of VR environments, there is still a need to further enhance focus-assisted methods to transfer 360° experiences more efficiently. 

% A review of 360° panoramic technology in architecture, engineering, and construction (AEC) points out problems in the application of 360° panoramic technology, motion sickness, splicing error effects, static viewpoints, and resolution problems\cite{shinde2023systematic}. 

% If combine our dataset, the binocular view provides deeper depth information and detail resolution, which is essential for creating more realistic and detailed virtual environments. Meanwhile, the third-person view provides the ability to view the scene from the outside, increasing the variety of perspectives and contributing to a more complete understanding of the scene. Additionally, this multi-view integration provides a more natural and rich visual fluidity, helping to reduce motion sickness issues in virtual reality environments while increasing user immersion and engagement. Also,it will benefit the areas that applied VR technology including education where virtual teaching tools are using\cite{bogusevschi2020teaching},virtual shopping in retail\cite{kim2022virtual}, and psychology field\cite{voigt2020comparing}.


% Our motivation is based on the finding that multi-view data can improve model understanding of the real-world scenarios \cite{girdhar2023imagebind}. 
 % After conducting thorough experiments, we are confident that our dataset has the potential to enhance models' comprehension by combining third-person and egocentric views of the surrounding environment. 


% Using the example of self-driving systems, current research can be broadly categorized into two directions: vehicle-side and infrastructure-side. While significant progress has been made in both areas, separately, there is still debates over current algorithms lacking in accuracy and efficiency \cite{yurtsever2020survey}. The  exploration of integrating these two perspectives is recognized as a potential 

% --------------------------------------
% Need for Granular Task Evaluation: To better understand the individual contributions of different views, i
\noindent{\bf \Rone Q\thenum: It would be valuable to evaluate tasks like TAL, with variations of views as in Table {\color{black} 2}.}
\vspace{0.1cm}


\noindent{\bf A:} As suggested, we further include experiments of variations of views for the Temporal Action Localisation (TAL) task, as detailed in Table \ref{table:TAL_extra}. The results therein show a trend consistent with those observed in Table {\color{black} 2}, indicating that the utilisation of multiple views contributes positively. 
% Furthermore, the integration of additional modalities is also shown to enhance performance. We will include these results in the final version.
\vspace{0.1cm}




\stepcounter{num}


% --------------------------------------
% (which is presented as a key characteristic of the dataset)
\noindent{\bf \Rone Q\thenum: The paper should elaborate more on the geographic distribution of the data collection. }
% Providing detailed statistics of this aspect (e.g., types action per location) would enhance the understanding of the dataset's diversity and applicability.}


% \noindent{\bf A\thenum:}
\input{rebuttal/location-action-dis}

\noindent{\bf A:}  As suggested, we further include  Fig. \ref{rebuttal:location-action}, to illustrate the `types action per location'. We can observe the geographic distribution and the diversity of the data, where the inner circle shows the location and the outer circle the action types captured in each location. 




% and the  This demonstrates that geographic data collections while the distribution of actions is location-specific.
% It aims to demonstrate the diversity and applicability of our dataset. \\
% We will incorporate this figure into the final version of the paper for a more comprehensive understanding.\\
\vspace{0.1cm}


\stepcounter{num}




% % --------------------------------------
% \noindent{\bf \Rone Q\thenum: request more granular evaluation on different scene understanding tasks.}


% % \noindent{\bf A\thenum:}
% \noindent{\bf A:}



% \stepcounter{num}


\vspace{1mm}
\setcounter{num}{1}
% --------------------------------------
\noindent{\bf \Rtwo Q: It would be better if some methodological innovation is included for the typical tasks.}
%  on the constructed dataset


\noindent{\bf A:} Thanks for the suggestion. We have tried to incorporate innovative strategies for modality fusion and dataset pre-training. As depicted in Fig. {\color{black}2} in the supp. mat., we integrated Clip Order and Pace Prediction as our self-supervised learning methods. In Fig. {\color{black}3}  in supp. mat., a new Hierarchical Attention mechanism was designed to fuse multiple modalities. We also explored alternative modality fusion approaches, such as direct concatenation of modalities, concatenation followed by a linear layer, concatenation followed by self-attention, and varied hierarchical structures of hierarchical attention. The performance of these fusion methods on Temporal Action Localisation is systematically compared and presented in Table \ref{table:TAL_ablation}, suggesting the effectiveness of our presented hierarchical attention approach.


% Our primary focus in this project is to enhance the dataset by introducing additional modalities and perspectives. While we recognize the potential of exploring innovative approaches for specific tasks, such as Temporal Action Localization, we have to defer this progress due to face limitations in terms of computational resources.




\input{rebuttal/table_TAL_extra}
\input{rebuttal/table_ablation}


\input{rebuttal/table_VideoMAE}



% \stepcounter{num}

\vspace{1mm}
\setcounter{num}{1}
% --------------------------------------
\noindent{\bf \Rthree Q: The baseline and backbone models, such as I3D, seem out-of-date.}

% \noindent{\bf A\thenum:}
\noindent{\bf A:}
We acknowledge that I3D may be considered outdated. We used it as it was widely adopted in video understanding tasks in the literature. In response, \textit{we further explore more contemporary Transformer-based} models, \eg VideoMAE [Tong et al. 2022], pretrained on the Kinetics dataset, akin to the I3D model setting in the main paper. Table \ref{table:VideoMAE} reports the performance on temporal action localisation using VideoMAE. Compared to the results in Table {\color{black} 3} (\ie the greyed line I3D in Table~\ref{table:VideoMAE}), Transformer shows better performance. Additionally, this experiment further validates the impact/benefits of various views and modalities. Due to the time constraints of the rebuttal phase, we were unable to pretrain VideoMAE on our dataset. However, we will incorporate these results in the final version.



\stepcounter{num}






==> rebuttal/location-action-dis.tex <==
% \begin{figure}[!t]
% \centering
% \includegraphics[height=0.15\textheight]{rebuttal/city-action-distribution.pdf}


% \caption{\small Location-action distribution.}

% \label{rebuttal:location-action}
% \end{figure}

\begin{wrapfigure}{r}{0.27\textwidth}[!t]
% \hspace{1.0cm}
\begin{center}
\vspace{-1.1cm}
\hspace{-0.65cm}
%  左下右上  38
  % \includegraphics[width=0.253\textwidth, trim=10 0 20 20, clip  ]{rebuttal/city-action-distribution.pdf}
  \includegraphics[width=0.3\textwidth, clip]{rebuttal/city-action-distribution.pdf}

\end{center}
% \vspace{-8mm}  
\vspace{-6mm}  
% \hspace{-0.65cm}
% \hspace{-1cm}
\caption{Geographic distribution.}
\label{rebuttal:location-action}
% \vspace{-3em}
\vspace{-1.5em}

\end{wrapfigure}




==> rebuttal/table_TAL_extra.tex <==




\begin{table}

	\centering
	% \caption{\small TAL results for different view combinations using TriDet, with extractors being \textit{I3D} pretrained on \textit{360+x}. The lines with a gray background were reported in the main paper.}
	\caption{\small TAL results for different views using TriDet, with extractors being \textit{I3D} pretrained on \textit{360+x}. The lines with a \textcolor{gray}{grey background} were reported in the main paper.}
    \label{table:TAL_extra}
	\small
\vspace{-0.3cm}

\resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}l|cccc|cccc|cccc@{}}
        \toprule
     
        \multirow{3}{*}{Selected View} & \multicolumn{4}{c}{V}& \multicolumn{4}{c}{V+A}& \multicolumn{4}{c}{V+A+D} \\
         & mAP & mAP & mAP & \multirow{2}{*}{Avg.\ }& mAP & mAP & mAP & \multirow{2}{*}{Avg.\ }& mAP & mAP & mAP & \multirow{2}{*}{Avg.\ }\\
         & $@$0.5 & $@$0.75 & $@$0.95 && $@$0.5 & $@$0.75 & $@$0.95 && $@$0.5 & $@$0.75 & $@$0.95 &\\
        
         \midrule
         
           \multirow{1}{*}{\makecell[c]{Egocentric Only}} &
     $ 12.5$ & $ 9.8$ & $4.3$ & $8.9$ \!\e{0.0}&$ 16.2$ & $ 12.3$ & $4.6$ & $11.0$ \!\e{0.0}&$ 16.9$ & $ 12.7$ & $4.7$ & $11.4$ \!\e{0.0}

 \\
            
           \multirow{1}{*}{\makecell[c]{Front Only}}  &
          $ 19.7$ & $ 14.4$ & $5.2$ & $13.1$ \!\p{4.2}&$ 24.5$ & $ 17.6$ & $6.1$ & $16.1$ \!\p{5.1}&$ 25.6$ & $ 18.0$ & $6.2$ & $16.6$ \!\p{5.2}
\\
             \cellcolor{gray!25} 
              \multirow{1}{*}{\makecell[c]{\du Only}} & \cellcolor{gray!25} 
        $ 21.1$ & \cellcolor{gray!25}  $ 15.3$ & \cellcolor{gray!25}  $5.5$ & \cellcolor{gray!25}  $14.0$ \!\p{5.1}& \cellcolor{gray!25} $ 26.4$ & \cellcolor{gray!25}  $ 18.5$ & \cellcolor{gray!25}  $6.9$ & \cellcolor{gray!25}  $17.3$ \!\p{6.3}& \cellcolor{gray!25} $ 27.1$ & \cellcolor{gray!25}  $ 18.7$ & \cellcolor{gray!25}  $7.0$ & \cellcolor{gray!25}  $17.6$ \!\p{6.2} 

        
        % { \multirow{1}{*}{\makecell[c]{\du Only}} &
        % $ 21.1$ & $ 15.3$ & $5.5$ & $14.0$ \!\p{5.1}&$ 26.4$ & $ 18.5$ & $6.9$ & $17.3$ \!\p{6.3}&$ 27.1$ & $ 18.7$ & $7.0$ & $17.6$ \!\p{6.2} }
\\
            
            
           \multirow{1}{*}{\makecell[c]{\du + Egocentric}} &
         $ 21.4$ & $ 15.8$ & $5.7$ & $14.3$ \!\p{5.4}&$ 27.3$ & $ 19.2$ & $7.2$ & $17.9$ \!\p{6.9}&$ 27.8$ & $ 19.6$ & $7.2$ & $18.2$ \!\p{6.8}
\\
            

            
           \multirow{1}{*}{\makecell[c]{\du + Front}} &
           $ 24.2$ & $ 16.8$ & $6.1$ & $15.7$ \!\p{6.8}&$ 28.1$ & $ 20.3$ & $7.3$ & $18.6$ \!\p{7.6}&$ 28.2$ & $ 20.8$ & $7.3$ & $18.8$ \!\p{7.4}
\\
            
            
           \multirow{1}{*}{\makecell[c]{\du + Front + Ego}} &
       \boldsymbol{  $ 24.6$ }& \boldsymbol{$ 17.1$} & \boldsymbol{$6.3$ }& \boldsymbol{$16.0$ }\!\textbf{\p{7.1}}& \boldsymbol{$ 28.2$} & \boldsymbol{$ 20.6$ }& \boldsymbol{$7.3$ }&\boldsymbol{ $18.7$ }\!\p{7.7}&\boldsymbol{$ 28.8$ }& \boldsymbol{$ 21.0$}& \boldsymbol{$7.4$ }&\boldsymbol{ $19.1$} \!\textbf{\p{7.7} 
\\}
            
           

     \bottomrule
    \end{tabular}
    }
    
\vspace{-0.2cm}
\end{table}






==> rebuttal/table_VideoMAE.tex <==



\begin{table}
	\centering
	% \caption{ \small TAL results  using TriDet with extractors being \textit{VideoMAE} pretrained on \textit{kinetics}. The first lines was reported in the main paper using \textit{I3D} extractor as reference.}
	\caption{ \small TAL using TriDet with extractors being \textit{Transformer-based} model pretrained on \textit{kinetics}. The \textcolor{gray}{greyed line} was reported in the main paper using \textit{I3D} extractor, for reference.}
    \label{table:VideoMAE}
	\small
\vspace{-0.3cm}

\resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}l|cccc|cccc@{}}
        \toprule
     
        \multirow{3}{*}{Selected View} & \multicolumn{4}{c}{V}& \multicolumn{4}{c}{V+A} \\
         & mAP & mAP & mAP & \multirow{2}{*}{Avg.\ }& mAP & mAP & mAP & \multirow{2}{*}{Avg.\ }\\
         & $@$0.5 & $@$0.75 & $@$0.95 && $@$0.5 & $@$0.75 & $@$0.95&\\
        
         \midrule
        

          \multirow{1}{*}{\textcolor{Gray}{\makecell[c]{\du Only}, with I3D}} &
 \textcolor{Gray}{$ 16.7$\!\e{0.0}} &  \textcolor{Gray}{$ 10.1$\!\e{0.0} }&\textcolor{Gray}{  $ 4.8$\!\e{0.0} }&\textcolor{Gray}{  $ 10.5$\!\e{0.0} }&\textcolor{Gray}{ $ 23.6$\!\e{0.0} }&\textcolor{Gray}{  $ 17.2$\!\e{0.0} }& \textcolor{Gray}{ $ 6.4$\!\e{0.0} }&  \textcolor{Gray}{$ 15.7$\!\e{0.0}} 

          \\

 \midrule
          
%            \multirow{1}{*}{\makecell[c]{Egocentric Only}} &
%   $ 5.6$\!\m{11.1} & $ 4.2$\!\m{5.9} & $ 2.7$\!\m{2.1} & $ 4.2$\!\m{6.4} &$ 10.3$\!\m{13.3} & $ 7.3$\!\m{9.9} & $ 3.9$\!\m{2.5} & $ 7.2$\!\m{8.6} 


%  \\
            
%            \multirow{1}{*}{\makecell[c]{Front Only}}  &
%           $ 16.2$\!\m{0.5} & $ 12.8$\!\p{2.7} & $ 4.8$\!\e{0.0} & $ 11.3$\!\p{0.7} &$ 24.0$\!\p{0.4} & $ 16.9$\!\m{0.3} & $ 5.6$\!\m{0.8} & $ 15.5$\!\m{0.2} 

% \\
            
 \multirow{1}{*}{\makecell[c]{\du Only}} &
 $ 17.1$\!\p{$0.4$} & $ 13.4$\!\p{$3.3$} & $ 5.2$\!\p{$0.4$} & $ 11.9$\!\p{$1.4$} &$ 25.9$\!\p{$2.3$} & $ 18.5$\!\p{$1.3$} & $ 6.1$\!\m{$0.3$} & $ 16.8$\!\p{$1.1$} 

 
 \\
        
        % { \multirow{1}{*}{\makecell[c]{\du Only}} &
        % $ 21.1$ & $ 15.3$ & $5.5$ & $14.0$ \!\p{5.1}&$ 26.4$ & $ 18.5$ & $6.9$ & $17.3$ \!\p{6.3}&$ 27.1$ & $ 18.7$ & $7.0$ & $17.6$ \!\p{6.2} }

            
            
           \multirow{1}{*}{\makecell[c]{\du + Egocentric}} &
       $ 16.9$\!\p{0.2} & $ 13.1$\!\p{3.0} & $ 5.0$\!\p{0.2} & $ 11.7$\!\p{1.1} &$ 26.4$\!\p{2.8} & $ 19.0$\!\p{1.8} & $ 6.2$\!\m{0.2}& $ 17.2$\!\p{1.5} 

\\
            

            
           \multirow{1}{*}{\makecell[c]{\du + Front}} &
           $ 19.5$\!\p{2.8} & $ 16.3$\!\p{6.2} & $ 5.6$\!\p{0.8} & $ 13.8$\!\p{3.3} &$ 27.6$\!\p{4.0} & $ 21.2$\!\p{4.0} & $ 6.5$\!\p{0.1} & $ 18.4$\!\p{2.7} 


          \\
            
            
           \multirow{1}{*}{\makecell[c]{\du + Front + Ego}} &
       \boldsymbol{$19.2$}\!\textbf{\p{2.5} }&\boldsymbol{$15.8$}\!\textbf{\p{5.7}}&\boldsymbol{$5.4$}\!\textbf{\p{0.6} }&\boldsymbol{$13.5$}\!\textbf{\p{2.9}}&\boldsymbol{$27.8$}\!\textbf{\p{4.2}}&\boldsymbol{$21.7$}\!\textbf{\p{4.5} }&\boldsymbol{$6.6$}\!\textbf{\p{0.2}}&\boldsymbol{$18.7$}\!\textbf{\p{3.0}}

\\
            
           

     \bottomrule
    \end{tabular}
    }
    
\vspace{-0.3cm}
\end{table}






==> rebuttal/table_ablation.tex <==



\begin{table}
	\centering
	% \caption{ \small TAL resultsusing TriDet, with extractors being \textit{I3D} pretrained on \textit{360+x}. The experiments are conducted under 360+Egocentric+F and V+A+D. The notation X$\to$Y represents X as the query and Y as the key-value pair in the attention mechanism.}
	\caption{ \small TAL with TriDet, \textit{I3D} pretrained on \textit{360+x}, under the setting 360+Egocentric+F and V+A+D. X$\to$Y: X as the query and Y as the key-value pair in the attention mechanism.}
    \label{table:TAL_ablation}
	\small
\vspace{-0.3cm}

\resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}l|cccc@{}}
        \toprule
     
        \multirow{1}{*}{Feature Fusion} 
        
         
         & mAP$@$0.5  & mAP$@$0.75  & mAP$@$0.95  & \multirow{1}{*}{Avg.\ }\\
         % & & & \\
        

 \midrule
          
 Concatenation&$ 19.2$\!\e{$0.0$} & $ 14.6$\!\e{$0.0$} & $ 5.3$\!\e{$0.0$} & $ 13.0$\!\e{$0.0$} \\
Concat + Linear Layer&$ 21.2$\!\p{$2.0$} & $ 15.1$\!\p{$0.5$} & $ 5.5$\!\p{$0.2$} & $ 13.9$\!\p{$0.9$}   \\
Concat + Self-Attention&$ 26.9$\!\p{$7.7$} & $ 18.9$\!\p{$4.3$} & $ 6.8$\!\p{$1.5$} & $ 17.5$\!\p{$4.5$}  \\
D$\to$V + Concat A&$ 17.8$\!\m{$1.4$}& $ 13.8$\!\m{$0.8$}& $ 5.2$\!\m{$0.1$}& $ 12.3$\!\m{$0.8$}\\
D$\to$A + Concat V&$ 24.6$\!\p{$5.4$} & $ 17.2$\!\p{$2.6$} & $ 6.2$\!\p{$0.9$} & $ 16.0$\!\p{$3.0$}   \\
A$\to$D + Concat V&$ 20.5$\!\p{$1.3$} & $ 14.9$\!\p{$0.3$} & $ 5.7$\!\p{$0.4$} & $ 13.7$\!\p{$0.7$}   \\
A$\to$V + Concat D&$ 28.3$\!\p{$9.1$} & $ 20.6$\!\p{$6.0$} & $ 7.3$\!\p{$2.0$} & $ 18.7$\!\p{$5.7$}  \\

\midrule

Hierarchical Attention, D$\to$A, A$\to$V&\boldsymbol{$28.8$}\!\textbf{\p{$9.6$}}&\boldsymbol{$21.0$}\!\textbf{\p{$6.4$}} &\boldsymbol{$7.4$}\!\textbf{\p{$2.1$}} &\boldsymbol{$19.1$}\!\textbf{\p{$6.0$}}

\\
            

            
           

     \bottomrule
    \end{tabular}
    }
    
\vspace{-0.2cm}
\end{table}





